Key Establishment in the Space Environment

As reliance on space systems continues to increase, so does the need to ensure security for them. However, public work in space standards have struggled with defining security protocols that are well tailored to the domain and its risks. In this work, we investigate various space networking paradigms and security approaches, and identify trade-offs and gaps. Furthermore, we describe potential existing security protocol approaches that fit well into the space network paradigm in terms of both functionality and security. Finally, we establish future directions for enabling strong security for space communication.

==> OpinionPaper/conclusions.tex <==
\section{Conclusions and Future Work}

% future work

% conclusions
